Detecting Small Query Graphs in A Large Graph via Neural Subgraph Search

Recent advances have shown the success of using reinforcement learning and search to solve NP-hard graph-related tasks, such as Traveling Salesman Optimization, Graph Edit Distance computation, etc. However, it remains unclear how one can efficiently and accurately detect the occurrences of a small query graph in a large target graph, which is a core operation in graph database search, biomedical analysis, social group finding, etc. This task is called Subgraph Matching which essentially performs subgraph isomorphism check between a query graph and a large target graph. One promising approach to this classical problem is the "learning-to-search" paradigm, where a reinforcement learning (RL) agent is designed with a learned policy to guide a search algorithm to quickly find the solution without any solved instances for supervision. However, for the specific task of Subgraph Matching, though the query graph is usually small given by the user as input, the target graph is often orders-of-magnitude larger. It poses challenges to the neural network design and can lead to solution and reward sparsity. In this paper, we propose NSUBS with two innovations to tackle the challenges: (1) A novel encoder-decoder neural network architecture to dynamically compute the matching information between the query and the target graphs at each search state; (2) A novel look-ahead loss function for training the policy network. Experiments on six large real-world target graphs show that NSUBS can significantly improve the subgraph matching performance.

==> sec-baseline.tex <==
\section{Baseline Description and Comparison}
\label{sec-baselines}

% \yba{describe all baselines in detail, focusing on neuralmcs, gwqap, pca -- we need to convince people our model in theory is better}

For all the models used in experiments, we evaluate their performance under the same search framework, i.e. with consistent search iteration counting, upper bound estimation, etc. \mcsp and \mcsprl use heuristics to select node pairs, which is ineffective as shown in the main text and has been described in Section~\ref{subsec-comp-search}. Therefore, this Section focuses on the comparison with the rest baselines, i.e. \gwqap~\citep{xu2019scalable}, \pca~\citep{wang2019learning}, and \mcstreemodel~\citep{bai2020neural}. 

% \subsection{\gwqap}

\gwqap is a state-of-the-art graph matching model for general graph matching. The task is not about MCS specifically, but instead about matching two graphs with its own criterion based on the Gromov-Wasserstein discrepancy~\citep{peyre2016gromov}. Therefore, we suppose the matching matrix $\bm{Y}$ generated for each graph pair can be used as a guidance for which node pairs should be visited first. In other words, we pre-compute the matching scores for all the node pairs before the search starts, and in iteration, we look up the matching matrix and treat the score as the $q$ score for action selection. \pca and \mcstreemodel essentially compute a matching matrix too, and it is worth mentioning that all the three methods cannot learn a score based on both the state and the action. They can be regarded as generating the matching scores based on the whole graphs only without being conditioned and dynamically updated on states and actions. 

\pca is a state-of-the-art image matching model, where each image is turned into a graph with techniques such as Delaunay triangulation~\citep{lee1980two}. It utilizes similarity scores and normalization to perform graph matching. We adapt the model to our task by replacing these layers with 3 GAT layers, consistent with \mcsrlmodel. As the loss is designed for matching image-derived graphs, we alter their loss functions to binary cross entropy loss similar to \mcstreemodel which will be detailed below.

\mcstreemodel is proposed for MCS detection with similar idea from \pca that a matching matrix is generated for each graph pair using GNNs. However, they both require the supervised training signals, i.e. the complete search for training graph pairs must be done to guide the update of \pca and \mcstreemodel. In contrast, \mcsrlmodel is trained under the RL framework which does not require the complete search (in stage 2 and 3, only sequences are generated as detailed in Section~\ref{subsec-tree-vs-seq}). This has the benefit of exploring the large action space in a ``smarter'' way and eventually allows our model to outperform \pca and \mcstreemodel. In implementation, the complete search is not possible for large training graph pairs, so instead we apply a search budget and use the best solution found so far to guide the training of \pca and \mcstreemodel.

Regarding the subgraph extraction strategy, for all the baselines, we use the same branch and bound algorithm, which is the state-of-the-art search designed for MCS~\citep{mccreesh2017partitioning}. However, as mentioned in Section~\ref{subsec-backtrack-dqn}, only our model is equipped with the ability to backtrack in a principled way. The main text shows the performance gain to \mcsrlmodel brought by the backtracking ability.

% \yba{TODO: theoretical time and memory complexity}




% We evaluate \mcstreemodel against the state-of-the-art solver, \mcsp, which uses heuristics and the branch and bound algorithm to achieve efficient computation for MCS. While the fastest among exact solvers, this method still has, in the worst case, exponential time complexity~\citep{mccreesh2017partitioning}. For this reason, in practice, its running time is much slower than the other approximate baselines. However, we still use \mcsp to generate ground-truth MCS results and it only takes a few days on a standard CPU server with multi-threading to handle all the ground-truth result generation.

% The representation learning baselines are adapted from recent graph matching techniques, specifically \cvpr~\citep{zanfir2018deep} and \pca (Permutation Loss and Cross-graph Affinity)~\citep{wang2019learning}. Both these methods utilize similarity scores and normalization to perform graph matching. As \cvpr uses CNN layers to form their node embeddings from images (with techniques such as Delaunay triangulation~\citep{lee1980two}), we adapt the model to our task by replacing these layers with 3 GAT layers, consistent with \mcstreemodel. \pca uses a node embedding mechanism similar to GMN, not requiring further adaptation. As the loss functions for both these methods were designed for image graphs, we alter their loss functions to binary cross entropy loss (the same as \mcstreemodel).

% We conduct the extraction process by first removing all nodes where its corresponding summation of similarity scores across rows or columns falls below a tuneable threshold (the values of which can be found in Appendix~\ref{sec-detail}) in the matching matrix, then selecting an equal number of nodes in both graphs. The latter is done by maximizing the similarity scores of uniquely selected node pairs through applying the Hungarian Algorithm~\citep{kuhn1955hungarian} on the remaining nodes of the matching matrix. This is because the extracted subgraphs, after just thresholding, may be of different sizes due to thresholding. The extra procedure ensures that we extract subgraphs of equal sizes and in addition, the Hungarian Algorithm yields one-to-one node-node correspondences for the extracted subgraphs. However, these methods do not necessarily result in isomorphic subgraphs.

% We also compare against two basic models, \basicgat~\citep{velickovic2017graph} and \basicgmn~\citep{li2019graph}, which use 3 GAT and GMN layers respectively to encode the initial node features, followed by similarity score computation. These baselines uses a simpler normalization scheme by appling element-wise sigmoid function ($y=1/(1+e^{-x})$) to the matching matrix, and directly feed the similarity matrix to the same loss function as defined by \mcstreemodel. \basicgat and \basicgmn use the same extraction method as the graph matching baselines.

% With exception to \mcsp, all these baselines run in polynomial time complexity with respect to the number of nodes in the two input graphs.

==> sec-dataset.tex <==
\section{Dataset Description}
\label{sec-dataset}

% \yba{TODO: emphasize they are large and real-world representative}

This section describes the datasets used for evaluating our model and baselines. Section~\ref{subsec-cur-learning} describes the dataset we use for training \mcsrlmodel as well as baseline learning based graph matching models.
% Anonymous. (2020). Maximum Common Subgraph Detection [Data set]. Zenodo. http://doi.org/10.5281/zenodo.3676334

% The datasets have been deposited in a data repository preserving anonymity~\cite{anonymous_2020_3676334} and can be found at \url{http://doi.org/10.5281/zenodo.3676334}. The code including the implementation of our model and the baseline methods as well as the code for graph generation are also available as part of the supplementary material submission.

We use the following real-world datasets for evaluation:
\begin{itemize}
    \item \nci: It is a collection of small-sized chemical compounds \citep{wale2008comparison} whose nodes are labeled indicating atom type. We form 100 graph pairs from the dataset whose average graph size (number of nodes) is 28.73.
    \item \road: The graph is a road network of California whose nodes indicate intersections and endpoints and edges represent the roads connecting the intersections and endpoints~\citep{leskovec2009community}. The graph contains 1965206 nodes, from which we randomly sample a connected subgraph of around 0.05\% nodes twice to generate two subgraphs for the graph pair $\ga=(\mathcal{V}_1,\mathcal{E}_1)$ and $\gb=(\mathcal{V}_2,\mathcal{E}_2)$. 
    % Without further description, all the datasets below use the same sampling strategy as \road.
    \item \kgen, \kgzh, and \kgenzh: It is a dataset originally used in a work on cross-lingual entity alignment~\citep{sun2017cross}. The dataset contains pairs of DBpedia knowledge graphs in different languages. For \kgen, we use the English knowledge graph and sample 10\% nodes twice to generate two graphs for our task. For \kgzh, we sample around 10\% nodes from the knowledge graph in Chinese. For \kgenzh, we sample once from the English graph to get $\ga$ and sample once from the Chinese graph to get $\gb$. Note that although the nodes have features, we do not use them because our task is more about graph structural matching rather than node semantic meanings, and leave the incorporation of continuous node initial representations as future work.
    \item \enron: The graph is an email communication network whose nodes represent email addresses and (undirected) edges represent at least one email sent between the addresses~\citep{klimt2004introducing}. From the total 36692 nodes, we sample around 10\% nodes to generate the graph pair.
    \item \amazon: An Amazon computer product network whose nodes represent goods and edges represent two goods frequently purchased together~\citep{shchur2018pitfalls}. The graph contains 703655 nodes from which we sample around 0.5\% to get the pair we use.
    \item \circuit: This is a graph pair 
    % provided by Mentor Graphics, 
    where each graph is a circuit diagram whose nodes represent devices/wires and edges represent the connecting relations between devices and wires. In other words, each node is either a device or a wire, and the entire graph is bipartite. The two graphs given are known to be isomorphic and we do not perform any sampling. Nodes have labels about the type of the device/wire. In real world, the successful matching of circuit layout diagrams is an essential process in circuit design verification.
    \item \ppi: It is a human protein-protein interaction network whose nodes represent proteins and edges represent physical interaction between proteins in a human cell~\citep{agrawal2018large}. From the 21557 nodes, we sample around ~10\% nodes to generate the pair used in experiments.
% Among all the datasets, the edges are undirected, and the only dataset with node labels is \circuit.

\end{itemize}
The details of all the graph pairs can be found in Table~\ref{table-test-data}. 



% \subsection{Details of Real Graph Datasets}

% \yba{TODO: describe}



\begin{table}[h]
% \small
  \begin{center}
    \caption{Details of real-world graph pairs used in evaluating the performance of baseline methods and \mcsrlmodel.}
    \begin{tabular}{l|lllllllll}
    \label{table-test-data}
      \textbf{Name} & \textbf{Description} & $|\mathcal{V}_1|$ & $|\mathcal{V}_2|$ & $|\mathcal{E}_1|$ & $|\mathcal{E}_2|$ & $\frac{|\mathcal{E}_1|}{|\mathcal{V}_1|}$ & $\frac{|\mathcal{E}_2|}{|\mathcal{V}_2|}$ \\
      \hline
      \textbf{\road} & Road Network & 1114 & 652 & 1454 & 822 & 1.305 & 1.261 \\
      \textbf{\kgen} & Knowledge Graph & 1945 & 1945 & 6242 & 5851 & 3.209 & 3.008 \\
      \textbf{\kgzh} & Knowledge Graph & 1907 & 1907 & 4856 & 4948 & 2.546 & 2.595 \\
      \textbf{\kgenzh} & Knowledge Graph & 1945 & 1907 & 6242 & 4856 & 3.209 & 2.546 \\
      \textbf{\enron} & Email Communication Network & 3369 & 3369 & 46399 & 50637 & 13.772 & 15.030 \\
      \textbf{\amazon} & Product Co-purchasing Network & 3518 & 3518 & 56028 & 40633 & 15.926 & 11.550 \\
      \textbf{\circuit} & Circuit Layout Diagram & 4275 & 4275 & 6128 & 6128 & 1.433 & 1.433 \\
      \textbf{\ppi} & Protein-Protein Interaction Network & 2152 & 2152 & 54910 & 54132 & 25.516 & 25.154 \\

    \end{tabular}
  \end{center}
% \vspace*{-6mm}
\end{table}


% \yba{Derek: Please rephrase text below to avoid self -copying. Also include only 2 out of the 4. Thanks!}

% We run experiments on 4 diverse different real world datasets coming from the chemical, programming language, and social network domains. For each dataset, we split the pairs into training, validation, and testing sets in the ratio of 6:2:2 such that none of the training, validation, or testing sets share any common graphs. For each dataset, we either one-hot encode node labels, if the dataset has node labels, or provide the same initial encoding, if the dataset does not have node labels. The code and the datasets have been published to this anonymous link: \url{https://github.com/openpublicforpapers/NeuralMCS}. 

% \subsubsection{\aids}% \yba{fix fonts}\derek{fixed.}
% \aids is a collection of antivirus screen chemical compounds, obtained from the Developmental Therapeutics Program at NCI/NIH\footnote{\url{https://wiki.nci.nih.gov/display/NCIDTPdata/AIDS+Antiviral+Screen+Data}}. The \aids dataset has been used by many works in graph matching~\citep{zeng2009comparing,wang2012efficient,zheng2013graph,zhao2013partition,liang2017similarity,bai2018graph}. These chemical compounds have node labels representing chemical elements (ex. Carbon, Nitrogen, Chlorine, and etc.) and edges denoting bonds between atoms. There are a total of 700 graphs, from which we sample 29610 graph pairs. The average graph size is 8.664 with the largest graph having 10 nodes.

% \subsection{\linux}
% \linux is a dataset of program dependence graphs (PDG) describing individual functions generated from the Linux kernel~\citep{wang2012efficient}. These graphs consist of unlabeled nodes and unlabeled edges, where nodes represent statements and edges represent control flow between statements. There are a total of 1000 graphs, from which we sample 60114 graph pairs. The average graph size is 7.591 and the largest graphs have 10 nodes.

% \subsection{\imdb}
% \imdb is a dataset of ego-networks of movie actors/actresses from the IMDB website~\citep{yanardag2015deep}. This dataset has been used by various works in graph classification~\citep{zhang2018capsule,bai2019unsupervised}. % \WW{fix the citation link} \derek{fixed}
% These graphs consist of unlabeled nodes and unlabeled edges, where nodes represent actors/actresses and edges represent whether they have had collaborations. There are a total of 1500 graphs, from which we sample 135702 graph pairs. The average graph size is 12.981 and the largest graphs have 89 nodes.

% \subsubsection{\reddit}
% \reddit is a collectionn of online dicussion networks from the Reddit online discussion website~\citep{yanardag2015deep}. The nodes in this dataset are unlabeled, where nodes represent users in a thread and edges represent whether users interactions in the discussion. Totally, there is 7112 graphs, from which we sample 3556 pairs. The average graph size is 11.8 nodes and the largest graph has 16 nodes.

For synthetic datasets, we generate graph pairs using the Barab{\'a}si-Albert (BA)~\citep{barabasi1999emergence} algorithm (edge density set to 5), the Erd\H{o}s-R{\'e}nyi (ER)~\citep{gilbert1959random} algorithm (edge density set to 0.08), and the Watts–Strogatz (WS)~\citep{watts1998collective} algorithm (rewiring probability set to 0.2 and ring density set to 4), respectively.

% ----------- ba -----------
% num_nodes: mean=50.0
% num_edges: mean=225.0
% avg_degree: 	mean=4.5
% ----------- ba100 -----------
% num_nodes: mean=100.0
% num_edges: mean=475.0
% avg_degree: 	mean=4.75
% ----------- er -----------
% num_nodes: mean=50.0
% num_edges: mean=101.79
% avg_degree: 	mean=2.0358
% ----------- er100 -----------
% num_nodes: mean=100.0
% num_edges: mean=395.15
% avg_degree: 	mean=3.9515
% ----------- ws -----------
% num_nodes: mean=50.0
% num_edges: mean=100.0
% avg_degree: 	mean=2.0
% ----------- ws100 -----------
% num_nodes: mean=100.0
% num_edges: mean=200.0
% avg_degree: 	mean=2.0

==> sec-dqn.tex <==
\section{Details on DQN and Training \mcsrlmodel}

\subsection{Training Data Preparation: Curriculum Learning}
\label{subsec-cur-learning}

Curriculum learning~\citep{bengio2009curriculum} is a strategy for training machine learning models whose core idea is to train a model first using ``easy'' examples before moving on to using ``hard'' ones. Our goal is to train a general model for MCS detection task which works well on general testing graph pairs from different domains. Therefore, we employ the idea of curriculum learning in training our \mcsrlmodel. More specifically, we prepare the training graph pairs in the following way:
\begin{itemize}
\item Curriculum 1: The first curriculum consists of the easiest graph pairs that are small: (1) We sample 30 graph pairs from \aids~\citep{zeng2009comparing}, a chemical compound dataset usually for graph similarity computation~\citep{bai2018graph} where each graph has less than or equal to 10 nodes; (2) We sample 30 graph pairs from \linux~\citep{wang2012efficient}, another dataset commonly used for graph matching consisting of small program dependency graphs generated from Linux kernel; (3) So far we have 60 real-world graph pairs. We then generate 60 graph pairs using popular graph generation algorithms. Specifcally, we generate 20 graph pairs using the BA algorithm, 20 graph pairs using the ER algorithm, and 20 graph pairs using the Watts–Strogatz WS algorithm, respectively. Details of the graphs can be found in Table~\ref{table-curriculum}. In summary, the first curriculum contains 120 graph pairs in total.
\item Curriculum 2: After the first curriculum, each next curriculum contains graphs that are larger and harder to match than the previous curriculum. For the second curriculum, we sample 30 graph pairs from \ptc~\citep{shrivastava2014new}, a collection of chemical compounds, 30 graph paris from \imdb~\citep{yanardag2015deep}, a collection of ego-networks of movie actors/actresses, and generate 20 graph pairs again using the BA, ER, and WS algorithms but with larger graph sizes.
\item Curriculum 3: For the third curriculum, we sample 30 graph pairs from \mutag~\citep{debnath1991structure}, a collection of chemical compounds, 30 graph paris from \reddit~\citep{yanardag2015deep}, a collection of ego-networks corresponding to online discussion threads, and generate 20 even larger graph pairs using the BA, ER, and WS algorithms.
\item Curriculum 4: For the last curriculum, we sample 30 graph pairs from \web~\citep{riesen2008iam}, a collection of text document graphs, 30 graph paris from \mcspconn~\citep{mccreesh2017partitioning}, a collection of synthetic graph pairs adopted by \mcsp, and generate 20 graph pairs again using BA, ER, and WS algorithms but with larger graph sizes.
\end{itemize}
For each curriculum, we train the model for 2500 iterations before moving on to the next, resulting in 10000 training iterations in total.

\begin{table}[h]
% \small
  \begin{center}
    \caption{Training graph details. For synthetic graphs, ``ed'', ``p'', and ``rd'' represent edge density, rewiring probability, and ring density, respectively.}
    \begin{tabular}{l|ll}
    \label{table-curriculum}
      \textbf{Curriculum} & \textbf{Data Source} & \textbf{\# Graph Pairs} \\
      \hline
      \multirow{5}{*}{\textbf{Curriculum 1}} & 
      \aids & 30 \\
      & \linux & 30 \\
      & BA:n=16,ed=5 & 20 \\
      & ER:n=14,ed=0.14 & 20 \\
      & WS:n=18,p=0.2,rd=2 & 20 \\
      \hline
     \multirow{5}{*}{\textbf{Curriculum 2}} & 
      \ptc & 30 \\
      & \imdb & 30 \\
      & BA:n=32,ed=4 & 20 \\
      & ER:n=30,ed=0.12 & 20 \\
      & WS:n=34,p=0.2,rd=2 & 20 \\
      \hline
     \multirow{5}{*}{\textbf{Curriculum 3}} & 
      \mutag & 30 \\
      & \reddit & 30 \\
      & BA:n=48,ed=4 & 20 \\
      & ER:n=46,ed=0.1 & 20 \\
      & WS:n=50,p=0.2,rd=4 & 20 \\
      \hline
     \multirow{5}{*}{\textbf{Curriculum 4}} & 
      \web & 30 \\
      & \mcspconn & 30 \\
      & BA:n=62,ed=3 & 20 \\
      & ER:n=64,ed=0.08 & 20 \\
      & WS:n=66,p=0.2,rd=4 & 20 \\
    \end{tabular}
  \end{center}
% \vspace*{-6mm}
\end{table}

% \subsection{Details of Graph Generation}
% \label{subsec-graph-generation}

% % \yba{Derek: Please introduce the detailed algorithms for BA, ER, and WS. Write as three formal algorithms.}

% As mentioned before, we adapt popular graph generation algorithms for generating graph pairs each sharing a common induced subgraph (common core) used as synthetic datasets. Therefore, for each graph pair, the MCS is at least as large as their common core, which can be used for evaluation as described in the main text. The challenge is to ensure the common core graph is subgraph isomorphic to both parent graphs while following the procedure of an underlying well-known graph generation algorithm. This section details the generation procedure with three underlying generation algorithm.

% We denote the graph pair to generate as $\mathcal{G}_1=(\mathcal{V}_1,\mathcal{E}_1)$ and $\mathcal{G}_2=(\mathcal{V}_2,\mathcal{E}_2)$. We denote the nodes of the common core as $\mathcal{V}_\alpha$, whose size is $K$, the nodes that are not in the common core as $\mathcal{V}_\beta$ and $\mathcal{V}_\gamma$ for $\mathcal{G}_1$ and $\mathcal{G}_2$ respectively. Thus, $\mathcal{V}_1$ is equivalent to $\mathcal{V}_\alpha \cup \mathcal{V}_\beta$, and $\mathcal{V}_2$ is equivalent to $\mathcal{V}_\alpha \cup \mathcal{V}_\gamma$. We denote the total number of nodes in the two graphs as N, i.e. $|\mathcal{V}_1|=|\mathcal{V}_2|=N$. We denote $\phi(\cdot)$ as a one-to-one function mapping one node from $\mathcal{V}_\beta$ to one node from $\mathcal{V}_\gamma$.

% Barab{\'a}si-Albert (BA)~\cite{barabasi1999emergence} generates graphs by successively adding and randomly connecting new nodes to the previously added nodes. In our case, we generate a graph pair by connecting the first $K$ nodes in the common core to the same previously added nodes, and then for the next $N-K$ nodes follow the BA framework independently. This is detailed in Algorithm~\ref{algo-ba}. We set the edge density (which is an integer) to 2 in the experiments.

% \begin{algorithm}[h!]
% 	\caption{Barab{\'a}si-Albert (BA) Graph Pair Generation}
% 	\begin{algorithmic}[1]
% 		\STATE \textbf{Input:} $K$, $N$, $density$.
% 		\STATE \textbf{Output:} $\ga$, $\gb$.
		
% 		\STATE Initialize $\ga \leftarrow (\O,\O)$.
% 		\STATE Initialize $\gb \leftarrow (\O,\O)$.
		
% 		\STATE $\mathcal{V}_\alpha \leftarrow K$ nodes.
% 		\STATE $\mathcal{V}_\beta \leftarrow N-K$ nodes.
% 		\STATE $\mathcal{V}_\gamma \leftarrow N-K$ nodes.
		
% 		\STATE \textbf{for} $v_\alpha \in \mathcal{V}_\alpha$
% 		    \STATE \quad $\mathcal{E}_s \leftarrow \O$
% 		    \STATE \quad \textbf{for} $i \in $ range$(density)$
% 		        \STATE \quad \quad Sample $v_s \in \mathcal{V}_1$
% 		        \STATE \quad \quad $\mathcal{E}_s.Insert((v_\alpha, v_s))$
% 		    \STATE \quad $\mathcal{V}_1.Insert(v_\alpha)$
% 		    \STATE \quad $\mathcal{V}_2.Insert(v_\alpha)$
% 		    \STATE \quad $\mathcal{E}_1.Extend(\mathcal{E}_s)$
% 		    \STATE \quad $\mathcal{E}_2.Extend(\mathcal{E}_s)$
		
% 		\STATE \textbf{for} $v_\beta \in \mathcal{V}_\beta$
% 		    \STATE \quad $\mathcal{E}_s \leftarrow \O$
% 		    \STATE \quad \textbf{for} $i \in $ range$(density)$
% 		        \STATE \quad \quad Sample $v_s \in \mathcal{V}_1$
% 		        \STATE \quad \quad $\mathcal{E}_s.Insert((v_\beta, v_s))$
% 		    \STATE \quad $\mathcal{V}_1.Insert(v_\beta)$
% 		    \STATE \quad $\mathcal{E}_1.Extend(E_s)$
		    
% 		\STATE \textbf{for} $v_\gamma \in \mathcal{V}_\gamma$
% 		    \STATE \quad $\mathcal{E}_s \leftarrow \O$
% 		    \STATE \quad \textbf{for} $i \in $ range$(density)$
% 		        \STATE \quad \quad Sample $v_s \in \mathcal{V}_2$
% 		        \STATE \quad \quad $\mathcal{E}_s.Insert((v_\gamma, v_s))$
% 		    \STATE \quad $\mathcal{V}_2.Insert(v_\gamma)$
% 		    \STATE \quad $\mathcal{E}_2.Extend(E_s)$
% 	\end{algorithmic}
% 	\label{algo-ba}
% \end{algorithm}


% Erd\H{o}s-R{\'e}nyi (ER)~\cite{gilbert1959random} generates graphs by randomly adding edges to $N$ isolated nodes where all edges have equal probability to be generated with an edge density parameter, $p$. In our case, we first generate the random core graph of $K$ nodes. Then, to ensure the newly added edges do not modify the already generated common core, for each new edge, we only add the edge if the two nodes in the edge are not in the common core graph. As this entire process does not ensure that the generated graphs are connected, we repeat it until $\mathcal{G}_1$, $\mathcal{G}_2$ and the common core graph are connected. This is detailed in Algorithm~\ref{algo-er}. We set $p$ to 0.07 in the experiments.

% \begin{algorithm}[h!]
% 	\caption{Erd\H{o}s-R{\'e}nyi (ER) Graph Pair Generation}
% 	\begin{algorithmic}[1]
% 		\STATE \textbf{Input:} $K$, $N$, $p$.
% 		\STATE \textbf{Output:} $\ga$, $\gb$.
		
% 		\STATE Initialize $\ga \leftarrow (\O,\O)$.
% 		\STATE Initialize $\gb \leftarrow (\O,\O)$.
		
% 		\STATE $\mathcal{V}_\alpha \leftarrow K$ nodes.
% 		\STATE $\mathcal{V}_\beta \leftarrow N-K$ nodes.
% 		\STATE $\mathcal{V}_\gamma \leftarrow N-K$ nodes.
		
% 		\STATE $\mathcal{V}_1 \leftarrow \mathcal{V}_\alpha \cup \mathcal{V}_\beta$
% 		\STATE $\mathcal{V}_2 \leftarrow \mathcal{V}_\alpha \cup \mathcal{V}_\gamma$
		
% 		\STATE \textbf{for} $e_s \in \mathcal{V_\alpha} \times \mathcal{V_\alpha}$
% 		    \STATE \quad \textbf{if} $random() < p$
% 		        \STATE \quad \quad $\mathcal{E}_1.Insert(e_s)$
% 		        \STATE \quad \quad $\mathcal{E}_2.Insert(e_s)$
        
% 		\STATE \textbf{for} $e_s \in \mathcal{V}_\beta \times (\mathcal{V}_\alpha \cup \mathcal{V}_\beta$)
% 		    \STATE \quad \textbf{if} $random() < p$
% 		        \STATE \quad \quad $\mathcal{E}_1.Insert(e_s)$

% 		\STATE \textbf{for} $e_s \in \mathcal{V}_\gamma \times (\mathcal{V}_\alpha \cup \mathcal{V}_\gamma$)
% 		    \STATE \quad \textbf{if} $random() < p$
% 		        \STATE \quad \quad $\mathcal{E}_2.Insert(e_s)$
		       
% 	\end{algorithmic}
% 	\label{algo-er}
% \end{algorithm}

% Watts–Strogatz (WS)~\cite{watts1998collective} generates graphs by starting with a ring lattice, a graph where each node is connected to a fixed number of neighbors, and then randomly re-wiring the edges of the lattice. In our case, we first generate $\mathcal{G}_1$ and $\mathcal{G}_2$ as two ring lattice graphs which are identical to each other. Then, we select $K$ nodes to be the common core, and perform rewiring on the two graphs ensuring the common core is subgraph isomorphic to $\mathcal{G}_1$ and $\mathcal{G}_2$. As this entire process does not ensure that the generated graphs are connected, we repeat it until $\mathcal{G}_1$, $\mathcal{G}_2$ and the common core graph are connected. This is detailed in Algorithm~\ref{algo-ws}. We set the ring density to 4 and the rewiring probability, $p$, to 0.2 in the experiments. We define the function $RingGraph(\mathcal{V},\theta)$ to simulate the process of creating a ring graph for $\mathcal{V}$ nodes connecting to $\theta$ neighbors on each side.

% % TODO: real dataset and then Imiation learning

% \begin{algorithm}[h!]
% 	\caption{Watts–Strogatz (WS) Graph Pair Generation}
% 	\begin{algorithmic}[1]
% 		\STATE \textbf{Input:} $K$, $N$, $RingDensity$, $p$.
% 		\STATE \textbf{Output:} $\ga$, $\gb$.
		
% 		\STATE $\mathcal{V}_\alpha \leftarrow K$ nodes.
% 		\STATE $\mathcal{V}_\beta \leftarrow N-K$ nodes.
% 		\STATE $\mathcal{V}_\gamma \leftarrow N-K$ nodes.

% 		\STATE $\ga = RingGraph(\mathcal{V}_\alpha \cup \mathcal{V}_\beta,RingDensity)$.
% 		\STATE $\gb = RingGraph(\mathcal{V}_\alpha \cup \mathcal{V}_\gamma,RingDensity)$.
		
% 		\STATE \textbf{for} $(v_i, v_j) $ such that $ v_i \in \mathcal{V}_\alpha, v_j \in \mathcal{V}_\alpha$
% 		    \STATE \quad \textbf{if} $random() < p$
% 		        \STATE \quad \quad Sample $v_{s1} \in \mathcal{V}_\alpha \cup \mathcal{V}_\beta$
% 		        \STATE \quad \quad Sample $v_{s2} = \phi(v_{s1})$
% 		        \STATE \quad \quad $\mathcal{V}_1.Remove((v_i, v_j))$
% 		        \STATE \quad \quad $\mathcal{V}_2.Remove((v_i, v_j))$
% 		        \STATE \quad \quad $\mathcal{V}_1.Insert((v_i, v_{s1}))$
% 		        \STATE \quad \quad $\mathcal{V}_2.Insert((v_i, v_{s2}))$
		
% 	    \STATE \textbf{for} $(v_i, v_j) \in \mathcal{E}_1$
% 		    \STATE \quad \textbf{if} $random() < p$
% 		        \STATE \quad \quad Sample $v_s \in \mathcal{V}_1$
% 		        \STATE \quad \quad \textbf{if} $v_i \notin \mathcal{V}_\alpha$ or $v_s \notin \mathcal{V}_\alpha$
%     		        \STATE \quad \quad \quad $\mathcal{E}_1.Remove((v_i, v_j))$
%     		        \STATE \quad \quad \quad $\mathcal{E}_1.Insert((v_i, v_s))$

% 	    \STATE \textbf{for} $(v_i, v_j) \in \mathcal{E}_2$
% 		    \STATE \quad \textbf{if} $random() < p$
% 		        \STATE \quad \quad Sample $v_s \in \mathcal{V}_2$
% 		        \STATE \quad \quad \textbf{if} $v_i \notin \mathcal{V}_\alpha$ or $v_s \notin \mathcal{V}_\alpha$
%     		        \STATE \quad \quad \quad $\mathcal{E}_2.Remove((v_i, v_j))$
%     		        \STATE \quad \quad \quad $\mathcal{E}_2.Insert((v_i, v_s))$

	    
		       
% 	\end{algorithmic}
% 	\label{algo-ws}
% \end{algorithm}


\subsection{Training Techniques and Details}
\label{subsec-train-details}

\subsubsection{Stage 1: Pre-training}
For the first 1250 iterations, we pre-train our DQN with the supervised true target $y_t$ obtained as follows: 
\begin{itemize}
\item For each graph pair, we run the complete search, i.e. we do not perform any pruning for unpromising states. The entire search space is explored, and the future reward for every action can be found by finding the longest path starting from the action to a terminal state. Since graphs are small in the initial stage, such complete search can be affordable. Using Figure 2 in the main text as an example, for the action that causes state 0 to transition to state 6, the longest path is 0, 6, 7, 11, 12, 13 (or 0, 6, 7, 11, 12, 14). 
\item Given the longest path found for each action, we then compute $y_t=1+\gamma+\gamma^2+...+\gamma^{(L-1)}$, where $\gamma$ is the discount factor set to 1.0, $L$ is the length of the longest path. In the example above, $y_t=5$, intuitively meaning that at state 0, for the action that leads to state 6, in future the best solution will have 5 more nodes. In contrast, the action 0 to 1 has $y_t=4$, meaning the action 0 to 6 is more preferred. 
\item Given the true target computed for each action, we run the mini-batch gradient descents over the mse loss $(y_t-Q(s_t,a_t))^2$, where the batch size (number of sampled actions) is set to 32. 
\end{itemize}


\subsubsection{Stage 2: Imitation Learning and Stage 3}

For stage 2 (2500 iterations) and stage 3 (6250 iterations), we train the DQN using the framework proposed in ~\citet{mnih2013playing}. The difference is that in stage 2, instead of allowing the model to use its own predicted $Q(s_t,a_t)$ at each state, we let the model make a decision using the heuristics by the \mcsp algorithm, which serves as an expert providing trajectories in stage 2. We aim to outperform \mcsp eventually after training using our own predicted $Q(s_t,a_t)$ in stage 3.
% rely on our own predicted $q_{ij}$ in stage 3


% We denote the DQN as a function $Q(s_t,a_t)$ which generates a q value for each state-action pair.
Here we describe the procedure of the training process. In each training iteration, we sample a graph pair from the current curriculum for which we run the DQN multiple times until a terminal state is reached to collect all the transitions, i.e. 4-tuples in the form of $(s_t,a_t,r_t,s_{t+1})$ where $r_t$ is 1
% if $s_{t+1}$ is a terminal state\footnote{The terminal state is when there is no more node pairs in connected bidomains, i.e. no more actions.} 
and $y_t = 1 + \gamma \max_{a'} Q(s_{t+1},a')$, and store them into a global experience replay buffer, a queue that maintains the most recent $L$ 4-tuples. In our calculations, $L=1024$. Afterwards, at the end of the iteration, the agent gets updated by performing the mini-batch gradient descents over the mse loss $(y_t-Q(s_t,a_t))^2$, where the batch size (number of sampled transitions from the replay buffer) is set to 32.



To stabilize our training, we adopt a target network which is a copy of the DQN network and use it for computing $\max_{a'} \gamma Q(s_{t+1},a')$. This target network is synchronized with the DQN periodically, in every 100 iterations.


Since at the beginning of stage 3, the q approximation may still be unsatisfactory, and random behavior may be better, we adopt the epsilon-greedy method by switching between random policy and Q policy using a probability hyperparameter $\epsilon$. Thus, the decision is made as $\argmax{\bm{q}}$ where $\bm{q}$ is the our predicted $Q(s_t,a_t)$ for all possible actions $(i,j)$ with $1-\epsilon$ probability; With $\epsilon$ probability, the decision is random. This probability is tuned to decay slowly as the agent learns to play the game, eventually stabilizing at a fixed probability. We set the starting epsilon to 0.1 decaying to 0.01.


% \subsubsection{Stage 3: Normal DQN Training}
% We adopt the standard Deep Q-learning framework~\citep{mnih2013playing}. For each $(\ga,\gb)$, the agent performs the subgraph exploration tree search, after which the parameters in the JSNE and DQN are updated. Notice each state is represented as a node in the subgraph exploration tree, and in each state, the agent tries to pick a new node pair. Since at the beginning of training, the q approximation is not well trained, and random behavior may be better, we adopt the epsilon-greedy method by switching between random policy and Q policy using a probability hyperparameter $\epsilon$. This probability is tuned to decay slowly as the agent learns to play the game, eventually stabilizing at a fixed probability. We set the starting epsilon to 0.7 decaying to 0.001.



% \subsection{Leveraging Labeled MCS Instances}

% As mentioned in the main text, the main advantage of \mcsrlmodel is that it does not require any labeled MCS instances, and thus can achieve better performane on larger graph datasets. It is noteworthy, however, that the subgraph exploration stage in \mcsrlmodel can naturally incorporate the ground-truth MCS results by extending the exploration tree into an exploration-imitation tree. This is accomplished by running the subgraph exploration procedure for a second time, where the initial pair selection is taken from the ground truth and on each iteration, only nodes from the ground truth can be selected, ultimately producing another imitation tree. As the ground truth may provide several correct sequences of node pair selections, we allow the $\beamsize$ of this second exploration-imitation tree to be tuned. This allows for more fine-grain tuning of exploration versus exploitation. By leveraging the labeled instances, the model can try better actions earlier on, improving the learning process. As shown in Table~\ref{table-il}, by incorporating the second imitation tree whose $\beamsize$ is also set to 5, we are able to achieve higher performance.

% \begin{table}[h!]
%   \begin{center}
%     \caption{Effect of using supervised data on the performance of \mcsrlmodel on \reddit.}
%     \begin{tabular}{l|l}
%       \textbf{Method} &
%       \textbf{Acc}
%     \\
%       \hline
% \mcstreemodel w/o sup & 93.187
% \\
% \mcstreemodel w sup & 95.934
% \label{table-il}
%     \end{tabular}
%   \end{center}
% \end{table}

\subsection{DQN Parameter Details}
\label{subsec-dqn-parameter-details}

% \yba{does Q reflect graph size? yes since sum rather than avg; then maybe in vis, we really show some Q on the gephi plot? but too many nodes hard to show...; initial local degree profile}

% \yba{justify the sum+MLP and 1dconv+MLP: without MLP just a global summation}

In experiments, we use $\textsc{sum}$ followed by an MLP for $\textsc{readout}$ and $\textsc{1dconv+maxpool}$ followed by an MLP for $\textsc{interact}$.  Specifically, the MLP has 2 layers down-projecting the node embeddings from 64 to 32 dimensions. Notice that different types of embeddings require different MLPs, e.g. the MLP used for aggregating and generating graph-level embeddings is different from the MLP used for aggregating and generating subgraph-level embeddings.

For $\textsc{1dconv+maxpool}$, we apply a 1-dimensional convolutional neural network to each one of two embeddings being interacted, followed by performing max pooling across each dimension in the two embeddings before feeding into an MLP to generate the final interacted embedding. Specifically, the $\textsc{1dconv}$ contains a filter of size 3 and stride being 1. The MLP afterwards is again a 2-layer MLP projecting the dimension to 32. As shown in the main text, such learnable interaction operator brings performance gain compared to simple summation based interaction. 

The final MLP takes four components, $\bm{h}_{\mathcal{G}} =\textsc{interact}(\bm{h}_{\mathcal{G}_1},\bm{h}_{\mathcal{G}_2})$, $\bm{h}_{s} =\textsc{interact}(\bm{h}_{s1},\bm{h}_{s2})$, $\bm{h}_{\mathcal{D}c}$, and $\bm{h}_{\mathcal{D}0}$, each with dimension 32. It consists of 7 layers down-projecting the 128-dimensional input ($32 \times 4$) to a scalar as the predicted $q$ score. For every MLP used in experiments, all the layers except the last use the $\mathrm{ELU}(x)$ activation function. An exception is the final MLP, whose last layer uses the $\mathrm{ELU}(x)+1$ as the activation function to ensure positive $q$ output.

A subtle point to notice is the necessity of using either nonlinear readout or nonlinear interaction for generating the bidomain representation. Otherwise, if both operators are a simple summation, the representation for all the connected bidomains ($\textbf{h}_{\mathcal{D}c}$) is essentially the global summation of all nodes in all the connected bidomains. In other words, the nonlinearity of MLP in the readout operation or the interaction operator allows our model to capture the bidomain partitioning information in $\textbf{h}_{\mathcal{D}c}$.

==> sec-future.tex <==
\section{Extensions of \mcsrlmodel}

\mcsrlmodel can be extended for a flurry of other MCS definitions, e.g. approximate MCS, MCS for weighted and directed graphs, etc. via a moderate amount of change to the search and learning components. In this section, we briefly outline what could be done for these tasks.

For approximate MCS detection, the bidomain constraint must be relaxed. One method of relaxing this constraint is to allow sets of nodes belonging to different but similar bidomains to match to each other. For instance, nodes in $\ga$ from the bidomain of bitstring ``00110'' could map with nodes in $\gb$  from the bidomain of bitstring ``00111'', since they are only 1 hamming distance away. Such relaxations as this can be made stricter or looser based on the application. The difference would be the search framework, thus the learning part of \mcsrlmodel can largely stay the same.

Regarding MCS for graphs with non-negative edge weights, assuming our task is to maximize the sum of edge weights in the MCS, instead of defining $r_t=1$, we can alter the reward function to be the difference of the sum of edge weights before and after selecting a node pair $r_t = \Sigma_{e \in S_t^{(u,v)}} w(e) - \Sigma_{e \in S_t} w(e)$ where $S_t$ is the edges of currently selected subgraph, $S_t^{(u,v)}$ is the edges of the subgraph after adding node pair, $(u,v)$, and $w(\cdot)$ is a function that takes and edge and returns its weight. As the cumulative sum of rewards at step T is the sum of edge weights $\Sigma_{t \in [1,...,T]} r_t = \Sigma_{e \in S_T} w(e)$ and reinforcement learning aims to maximize the cumulative sum of rewards, we can adapt GLSearch to optimize for MCS problems with weighted edges.

Regarding MCS for directed graphs, the bidomain constraint may be altered such that every bit in the bidomain string representations now has 3 states: `0' for disconnected, `1' for connected by in-edge, and `2' for connected by out-edge. By considering the inward/outward direction of a bitstring, we can guarantee the isomorphism of directed graphs. In this case, the search framework would only differ in how bidomains are partitioned. The learning part of GLSearch would stay the same for this application.

More generally, we believe that there are many more extensions to GLSearch in addition to the ones listed, such as disconnected MCS, network alignment, or subgraph extraction. Further exploration of these are to be done as future efforts.



==> sec-learn.tex <==
\section{Discussion on Learning Capacity of \gse}
\label{sec-learn}

In our current model, we form a matching matrix for both training and inference, and perform our loss function on the matching matrix during training (Section~\ref{subsec-learning}), and utilize GSE (Section~\ref{subsec-gse}) guided by the matching matrix during inference to extract subgraphs. We use GMN for node embeddings (Section~\ref{subsec-gmn} and Section~\ref{subsec-mmg}) and feed the matching matrix into GSE, which is fixed during the iterative GSE process. However, one potential issue is that once a node pair is selected, the extracted subgraph grows by one node causing the candidate pairs to change in the next iteration. Ideally, node embeddings should be updated to reflect such change after each iteration. By introducing learnable components to iteratively update the node embeddings to reflect such change, we can train the GSE component using guidance from the ground-truth node mappings in the MCS, making the training stage and inference stage consistent and match each other.

To accomplish this, we propagate the node embeddings at each iteration of GSE with learnable weights to recompute the matching matrix $\bm{Y}$ such that the next iteration's node embeddings will be conditionally updated based on the current extracted subgraph. To achieve it, we extend GMN to update the node embeddings for the extracted subgraph at each GSE iteration. GMN updates the node embeddings of two graphs jointly by performing intra- and inter-graph message passing. Thus, one can directly apply GMN to the extracted subgraph at each GSE iteration, and calculate the loss function at the end of GSE process (replacing the current BCE loss on the matching matrix $\bm{Y}$), achieving conditional node embeddings in the GSE step of the model. 

In implementation, we make a further modification to GMN by not propagating to matched nodes in the two extracted subgraphs. This is because we want the node embeddings for the currently extracted isomorphic subgraphs to stay as consistent as possible and not be influenced by any unpicked nodes in the larger graph or any nodes from the opposing graph.

We run both modified versions (with and without further modification) of \mcstreemodel on \aids, and the performance increase is only marginal ($<1\%$ increase). Therefore, by forgoing this step during training and only using GSE only during testing, we can gain a free speed up in training time.



% There are many promising directions, built on this idea of merging an iterative node selection procedure with a graph neural network-based selection criterion, to explore. First, we plan to further improve our model by introducing additional learnable components between selection steps, allowing for updates to the matching matrix between steps as we expand the search frontier. Second, we plan on using less computationally expensive isomorphism checks or using these checks more periodically to improve the speed of the model. Third, we plan to extend the search by incorporating the beam search~\citep{schwartz1990n} methodologies, where multiple search paths are explored simultaneously in a computationally efficient way. Fourth, we plan on introducing learnability to the subgraph embedding stopping condition to better help the model decide when to stop.

% These improvements are possible because the entire extraction process is differentiable. We can accomplish this by substituting the Gumbel softmax~\citep{jang2016categorical} in place of argmax for the node pair selection criterion and find the neighboring nodes through manipulation of the graphs' adjacency matrices.

% In future, another promising direction is to further test \mcstreemodel on very large-scale graph datasets, both with more pairs and larger individual graphs, e.g. \alchemy~\citep{chen2019alchemy}. First, one can utilize graph coarsening/pooling~\citep{ying2018hierarchical} to organize graphs in a hierarchy so that the model time complexity may be reduced. Second, the multiple choice learning components are executed sequentially, but in the future can be implemented to run in parallel through multi-threading to achieve even greater time reduction.
 
%\yba{i guess we also really need a section talking about future directions: (edited) 
%1. RNN methods ongoing
%2. the real search with beam size, budget, branch-and-bound heuristics
%in other words, we are NOT searching anything; we are just expanding by following a matrix (edited) 
%we need some good words to defend such potential critism}

==> sec-result.tex <==
\section{More Results with Analysis}
\label{sec-more-results}

\subsection{Number of Solved Pairs Across Time}

\begin{figure}
\vspace*{-4mm}
     \centering
     \subfloat[\textbf{\human $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/human-32.png}}
     \subfloat[\textbf{\human $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/human-64.png}}
     \subfloat[\textbf{\human $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/human-128.png}}
\vspace*{-3mm}
     \centering
     \subfloat[\textbf{\hprd $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/hprd-32.png}}
     \subfloat[\textbf{\hprd $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/hprd-64.png}}
     \subfloat[\textbf{\hprd $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/hprd-128.png}}
\vspace*{-3mm}
%      \centering
%      \subfloat[\textbf{\dblp $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{dblp-32.png}}
%      \subfloat[\textbf{\dblp $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{dblp-64.png}}
%      \subfloat[\textbf{\dblp $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{dblp-128.png}}
% \vspace*{-3mm}
     \centering
     \subfloat[\textbf{\eu $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/eu2005-32.png}}
     \subfloat[\textbf{\eu $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/eu2005-64.png}}
     \subfloat[\textbf{\eu $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/eu2005-128.png}}
\vspace*{-3mm}
     \centering
     \subfloat[\textbf{\youtube $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/youtube-32.png}}
     \subfloat[\textbf{\youtube $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/youtube-64.png}}
     \subfloat[\textbf{\youtube $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/youtube-128.png}}
     \caption{Comparison of the curves of the number of solved pairs versus time on \human, \hprd, \eu, and \youtube. The plot for \dblp are shown in the main text.}
     \label{fig:all-curves}
% \vspace*{-3mm}
\end{figure}

We provide figures on the number of solved pairs across time for all datasets in Figure~\ref{fig:all-curves}, showing that \sgmrlmodel consistently solves more query graph pairs than baseline methods on most datasets. Figure~\ref{fig:all-curves} also shows \sgmrlmodel's scalability with respect to query graph size, as baselines rapidly fail while \sgmrlmodel retains solid performance as query graphs get larger. Furthermore, the number of solutions found by baseline methods tend to flatten unlike \sgmrlmodel, which consistently solves more and more queries over time, suggesting that \sgmrlmodel will further outperform baselines if run for longer. We observe no clear correlation between the density of a query graph and the difficulty of solving the graph pair, i.e. the number of solutions found by the methods tested in our paper. We conjecture the difficulty is related to the distribution of the node degrees of a query graph, and leave the further investigation of predicting the difficulty of a graph pair without actually running a \task solver as future work.

\subsection{Results on Running Time}

We observe that the baseline solvers written in C++ have $O(1)$ time complexity for its random node selection policy for nodes in $G$, and thus tend to perform many more iterations than \sgmrlmodel written in Python during inference time.
% We report the total number of iterations and average running time per iteration for the methods tested in the main text. Since the baseline solvers are written in C++, and a fast random policy is adopted, they are much faster than \sgmrlmodel. 
However, even with many more iterations performed by these baselines, they still fail to solve most pairs due to the too large action space incurred by the 128-node query graphs. Although 128 nodes do not seem to be very large, due to the combinatorial nature of \task, the search space is still intractable for these fast baselines. In contrast, our model written in Python is slower for each iteration but offers a much better overall result, suggesting good practicality and the promising research direction of designing learning-based strategy to enhance search algorithms.

% \begin{table}[h]
% % \footnotesize
%   \begin{center}
%     \caption{Running time comparison on \dblp $Q_{128}$. The number of iterations is the averaged across the 100 pairs. ``ns'', ``ms'' denote nanoseconds and millisecond respectively. \yba{maybe just mention millions of iterations at high level}
%     }

    
%     \begin{tabular}{l|p{2.5cm}p{3cm}p{2cm}}
%     \label{table-timing}
%     \textbf{Model} & \textbf{\% Solved Pairs} & \textbf{\# Iterations} & \textbf{Time per Iter}\\
%     \hline
    
%     \qsi & 0.07 & 1092713998.89 & 274.55 ns \\ 
%     \gql & 0.02 & 459639.11 & 0.65 ms \\ 
%     \ceci & 0.18 & 1215745130.39 & 246.76 ns \\ 
%     \daf & 0.16 & 824427531.89 & 363.89 ns\\ 
%     \hybrid & 0.04 & 1928269226.84 & 155.58 ns \\ 
%     \nmatch & 0.04 & 24248.43 & 12.37 ms\\ 
    
%     \sgmrlmodel & \textbf{0.58} & 1724.06 & 174.01 ms\\ 
    
    
%     \end{tabular}
%   \end{center}
% % \vspace*{-4mm}
% \end{table}

We analyze the running time by showing the percentage of the major components in \sgmrlmodel. As shown in Figure~\ref{fig:pie}, without caching the intra-graph node embeddings, the propagation module is the bottleneck, due to its $\mathcal{O}(|E_q|+|E_G|)$ time complexity. It is noteworthy that we perform the propagation and matching modules sequentially to generate Figure~\ref{fig:pie} (a), i.e. for each \encoderlayer, we first run the propagation module and then run the matching module. Although it is possible to further optimize the implementation by running two modules in parallel (to be specific, the propagation module of layer $k$ and the matching module of layer $k-1$ could be performed in parallel on two devices), we argue the bottleneck would still be the propagation module, for which the proposed caching technique would help. In comparison, by caching the state-independent $\bm{h}_{\mathrm{intra}}^{(k)}$ node embeddings, the propagation module only takes $0.3\%$ (corresponding to the almost invisible slice of red color) of the total running time budget (5 minutes). 

\begin{figure}[h]
% \vspace*{-4mm}
     \centering
     \subfloat[\sgmrlmodel without caching of $\bm{h}_{\mathrm{intra}}^{(k)}$.]{\includegraphics[width=0.5\textwidth]{visualizations/pie_eu_no_caching.pdf}}
     \subfloat[\sgmrlmodel with caching of $\bm{h}_{\mathrm{intra}}^{(k)}$.]{\includegraphics[width=0.5\textwidth]{visualizations/pie_eu_caching.pdf}}
     \caption{Running time breakdown by executing \sgmrlmodel (the inference stage) on one randomly sampled graph pair from \eu for 5 minutes and collecting the running time spent on each component. With caching, more iterations are performed due to each iteration being much faster.}
     \label{fig:pie}
% \vspace*{-2mm}
\end{figure}


% \yba{also show CS and LCS changes across search iterations}
% \yba{mention average running time per iter?}

We plot the change of global candidate space (CS) size and the local candidate space (LCS) size across time in Figure~\ref{fig:cs-lcs}. Specifically, at each search iteration, a node $u_t$ from the query graph is chosen by $\phi$ (line 7 of Algorithm 1 in the main text), and the local candidate space is computed for $u_t$ (line 8 of Algorithm 1 in the main text). Therefore, we can record the number of candidates for $u_t$ in the global candidate space and in the local candidate space, and plot the change of CS and LCS sizes across search iterations. As shown in Figure~\ref{fig:cs-lcs}, there is a large reduction of candidate nodes from CS to LCS, suggesting the importance of computing a smaller local candidate space based on the current matching and the selected $u_t$. Without any LCS computation technique, the action space would be the global CS, which may contain up to $100,000$ nodes. Another important observation is that, the number of local candidate nodes varies dramatically across iterations. For example, in the initial iteration, since no nodes are matched, LCS is of the same size as CS, but as soon as one node pair is matched, the LCS computation can leverage the matched nodes by narrowing down the action space from all the nodes in CS to the first-order neighbors of the matched nodes. Existing LCS computation has several other techniques to reduce the candidate space size other than simply using the first-order neighbors of the matched subgraphs, and as a result, there can be less than 10 nodes in $\mathcal{A}_{u_t}$ in some iterations. However, when the search backtracks to an earlier state, there can be more candidate nodes in LCS, resulting in the varying LCS sizes across search.

\begin{figure}[h]
% \vspace*{-4mm}
     \centering
     \subfloat[\textbf{\human}]{\includegraphics[width=0.33\textwidth]{visualizations/human-cs.png}}
     \subfloat[\textbf{\hprd}]{\includegraphics[width=0.33\textwidth]{visualizations/hprd-cs.png}} \\
     \subfloat[\textbf{\dblp}]{\includegraphics[width=0.33\textwidth]{visualizations/dblp-cs.png}}
    \subfloat[\textbf{\eu}]{\includegraphics[width=0.33\textwidth]{visualizations/eu-cs.png}}
    \subfloat[\textbf{\youtube}]{\includegraphics[width=0.33\textwidth]{visualizations/youtube-cs.png}}
     \caption{Demonstration of the sizes of global candidate space (CS) and local candidate space (LCS) across search iterations, by running \sgmrlmodel on a randomly sampled graph pair from each dataset, and collecting the size of CS and LCS at each search iteration. The y-axis is in the log scale. We stop recording the CS and LCS sizes after 1000 search iterations.}%\yba{TODO: fix plots}}
     \label{fig:cs-lcs}
% \vspace*{-2mm}
\end{figure}

Since Figure~\ref{fig:cs-lcs} only shows the change of CS and LCS sizes across search for one graph pair, we show the statistics of CS and LCS sizes across 100 graph pairs in Table~\ref{table-cslcsstas}. Consistently with Figure~\ref{fig:cs-lcs}, the LCS size is on average smaller than the CS size, suggesting the importance of LCS computation.

\begin{table}[h]
% \footnotesize
  \begin{center}
    \caption{Statistics of the sizes of CS and LCS over 100 graph pairs for each dataset. ``Avg'', ``Min'', and ``Max'' denote average, minimum, and maximum, respectively.
    }
    
    \begin{tabular}{l|p{2cm}p{2cm}p{2cm}}
    \label{table-cslcsstas}
    \textbf{Dataset Name} & \textbf{Avg} & \textbf{Min} & \textbf{Max}\\
    \hline
    \textbf{\human $Q_{128}$ (CS)}  & 2217.65 & 395 & 4103 \\ 
    \textbf{\human $Q_{128}$ (LCS)}  & 55.65 & 0 & 1937 \\ \hline 
    \textbf{\hprd $Q_{128}$ (CS)}  & 4436.42 & 358 & 9031 \\ 
    \textbf{\hprd $Q_{128}$ (LCS)}  & 25.03 & 0 & 1911 \\ 
    \hline 
    \textbf{\dblp $Q_{128}$ (CS)}  & 170010.07 & 5370 & 317071 \\ 
    \textbf{\dblp $Q_{128}$ (LCS)}  & 23.34 & 0 & 62127 \\ 
    \hline 
    \textbf{\eu $Q_{128}$ (CS)}  & 612683.85 & 23327 & 861758 \\ 
    \textbf{\eu $Q_{128}$ (LCS)}  & 337.65 & 0 & 623730 \\ 
    \hline 
    \textbf{\youtube $Q_{128}$ (CS)}  & 368211.15 & 13248 & 1134773 \\
    \textbf{\youtube $Q_{128}$ (LCS)}  & 55.79 & 0 & 118752 \\
     
    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table}



% \yba{also mention batch operation for Q+U?}

\subsection{Results on Adapting \mcsrlmodel for \task}
\label{subsec=glsearchforsgm}

We report the performance of \sgmrlmodel and \mcsrlmodel on \task. As mentioned in Section~\ref{sec-related}, \task contains a tighter set of constraints than MCS, causing \mcsrlmodel's search framework to be less efficient and rely on a value-based model instead of a policy-based model. To measure the effects of both search framework and model design, we compare \sgmrlmodel to two models: (1) \mcsrlmodel, which uses the MCS search framework to conduct \task, and (2) \mcsrlmodeladapted, which uses the same value-based model architecture as \mcsrlmodel but adapted into \sgmrlmodel's search framework. To ensure the efficiency of value-based models, which need to execute an action before computing the $Q$ score, we adopt a simple sampling-based approach, where \mcsrlmodeladapted will always choose the best action out of up to 100 actions, regardless of the total action space size. We observe without such sampling, the model spends minutes executing a single action. Our results from Table~\ref{table-glsearch} emphasizes the differences between \task and MCS by confirming the criticality of \task search constraints and \sgmrlmodel's effective policy model design to \task performance.

\begin{table}[h]
% \footnotesize
\begin{center}
    \caption{Results of directly applying and adapting \mcsrlmodel originally designed for MCS detection to \task.}

    
    \begin{tabular}{l|lll}
    \label{table-glsearch}
    \textbf{Model} & \textbf{\dblp $Q_{32}$} & \textbf{\dblp $Q_{64}$} & \textbf{\dblp $Q_{128}$} \\
    \hline
    \sgmrlmodel & \textbf{1.00} & \textbf{0.97} & \textbf{0.58} \\ \hline
    \mcsrlmodel & 0.0 & 0.0 & 0.0 \\
    \mcsrlmodeladapted & 0.93 & 0.47 & 0.0 \\ 

    
    \end{tabular}
% \vspace*{-4mm}
\end{center}
\end{table}


\subsection{Reproducibility of Results}

We run the trained \sgmrlmodel model for 3 times to study the expected variance in model performance, due to the fixed running time budget used in experiments, and the fact that \sgmrlmodel tends to solve more pairs towards the end of the 5-minute budget for each pair as shown in Figure~\ref{fig:all-curves}. We find that \sgmrlmodel is able to reliably achieve good results on all datasets and outperform baseline methods. In contrast, baseline solvers in C++ tend to plateau and stop finding solutions for more pairs early in the 5-minute duration as seen in Figure~\ref{fig:all-curves}.

\begin{table}[h]
% \small
\footnotesize
  \begin{center}
    \caption{Reproducibility of the solved percentage results on the $Q_{128}$ datasets.
    }

    
    \begin{tabular}{l|ll}
    \label{table-acc}
    \textbf{Dataset} &\textbf{Mean} & \textbf{Stdev} \\
    \hline
    
    \textbf{\human $Q_{128}$} & 0.53 & 0.09 \\ 
    \textbf{\hprd $Q_{128}$} & 0.00 & 0.00 \\ 
    \textbf{\dblp $Q_{128}$} & 0.62 & 0.03 \\ 
    \textbf{\eu $Q_{128}$} & 0.23 & 0.03 \\
    \textbf{\youtube $Q_{128}$} & 0.11 & 0.01 \\ 
    
    % \textbf{\human $Q_{128}$} & 0.43 & 0.52* & 0.58* \\ 
    % \textbf{\hprd $Q_{128}$} & 0.00 & 0.00* & 0.00* \\ 
    % \textbf{\dblp $Q_{128}$} & 0.58 & 0.66 & 0.64 \\ 
    % \textbf{\eu $Q_{128}$} & 0.21 & 0.32* & 0.34* \\
    % \textbf{\youtube $Q_{128}$} & 0.11 & 0.10* & 0.14* \\ 
    
    % \hline
    
    % \textbf{\patents $Q_{32}$} & \textbf{0.78} & 0.16 & 0* & 0.67 & 0.19 & 0.20 & 0.52 \\ 
    % \textbf{\patents $Q_{64}$} & 0.54 & 0.27 & 0.00 & \textbf{0.64} & 0.00 & 0.31 & 0.61 \\ 
    % \textbf{\patents $Q_{128}$} & \textbf{0.24} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00** & 0.03 \\ 

    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table}



\subsection{Results on Labeled Graphs for \task}

To test the generality of \sgmrlmodel, we compare it against baselines on a labeled dataset. By assigning labels, the filtering algorithm can further reduce the search space prior to the search process. Because of this, labeled datasets are generally easier than unlabeled datasets. The degree to which labels make \task easier is hard to determine. For instance, if all the target graph nodes in the same global candidate set share the same label, then the additional label constraint provides little guidance to search. On the other extreme, if each query graph node has a unique label that matches only one target graph node, then the search becomes trivial. For example, Knowledge Graph (KG) reasoning~\cite{ren2020query2box,zhang2021cone} can also be viewed as matching a subgraph in a large KG, where a first-order logical query is represented as directed acyclic graph. However, since the KG can be incomplete with missing relations, exact \task may not be the most appropriate choice~\cite{ren2020query2box}.

To be fair, we adopt the labeled \eu dataset provided by \cite{sun2020memory} for our experiment, where $|\Sigma|=10$. Note, we do not retrain \sgmrlmodel on the labeled dataset, opting to use the same model trained on the unlabelled dataset. While node labels are not reflected in the initial features of the graph, they do shrink the size of the global and local candidate set, as only nodes with the same label can match eachother.%\yba{how do we handle node labels in CS or LCS?}

\begin{table}[h]
\begin{center}
% \footnotesize
    \caption{Results on labeled \eu-labeled $Q_{32}$ dataset. The ratio of the number of solved pairs over the 100 pairs is reported.
    }

    
    \begin{tabular}{l|p{2cm}}%
    \label{table-labeled}
    \textbf{Model} & \textbf{\eu-labeled $Q_{32}$} \\
    \hline
    
    \qsi & 0.35 \\ 
    \gql & 0.72 \\ 
    \ceci & 0.70 \\ 
    \daf & 0.86 \\ 
    \hybrid & 0.82 \\ 
    % \nmatch & 0.08 \\ 
    \sgmrlmodel & \textbf{0.99} \\
    \end{tabular}
% \vspace*{-4mm}
\end{center}
\end{table}

As seen in Table\ref{table-labeled}, \sgmrlmodel outperforms baselines even on labeled graph instances, demonstrating its generality. This suggests the graph structure is very critical in \task search algorithms, even in the presence of other constraints such as node labels. We also tried such experiments on smaller datasets provided by \cite{sun2020memory}, but found all methods were able to solve the graph pairs. As seen in Table~\ref{table-cslcsstas}, adding node labels to graphs with already small candidate sets could drastically reduce the search space, such that search space pruning on its own is enough to find a valid solution; however, as we have demonstrated thus far, there are many non-trivial cases where a smarter search policy, such as \sgmrlmodel, is required for \task. It is also possible to further improve \sgmrlmodel performance by training it on the labeled dataset, but we leave this as future work.






% \subsection{Results on Finding All the Solutions for \task}
% \yba{mention limitation: can be faster}
% \yba{future directions: Parallelism? Even larger target graphs? Subgraph search in a database? Build an index?}

% \subsection{Results on Generalization of Trained Models}



% \subsection{Best Solution Sizes across Time}

% % \yba{TODO: running time on circuit (address running DVN too slow; time complexity; in practice can even use CPP with parallel to further speed up; overall training one day but can be applied to all testing pairs); KL}

% Figure~\ref{fig-iter-size} shows that under the budget we set, for the large real-world graph pairs, all the methods reach a ``steady state'' where the best solution found so far no longer grows. This means the search continues but the search cannot find a larger solution, illustrating the fact that search gets ``stuck''. In theory, given infinitely many iterations, all the models will eventually find the true MCS, which is the largest, but since the task is NP-hard, the search space can be exponential in the worst case (subject to pruning but in all the testing graph pairs the search has not finished yet), such budget has to be applied to search. 
% % This also illustrates the motivation for our backtracking using DQN outputs as detailed in Section~\ref{subsec-backtrack-dqn}.
% At the end of the 7500 iterations, though, all the models have made ``mistakes'' (visiting unpromising states) and in order to find even larger common subgraphs, the search needs to backtrack potentially many times to fix those ``mistakes'' (backtracking to a very early state). 
% % Since all methods will eventually find the same true MCS given infinitely many iterations, 

% Admittedly, there is always the possibility that for more iterations, some baseline method may find a larger solution. Besides, in each iteration \mcsrlmodel does take more running time overhead as shown in Table~\ref{table-additional-runtime}. However, the point of our model is to quickly find a larger solution in as few iterations as possible, not to find a large solution given too many iterations. In other words, the goal of \mcsrlmodel is to be \textbf{smart} enough to \textbf{quickly} find a large solution instead of purely finding a good solution. Figure~\ref{fig-iter-size} shows that \mcsrlmodel not only finds solutions larger than baselines \textit{when} the 7500 iterations budget is reached but also finds larger solutions faster than baselines \textit{before} the budget is reached.


% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Average running time per iteration (msec).}
%     \begin{tabular}{l|llllllll}
%     \label{table-additional-runtime}
%     \textbf{Method}&
%     \textbf{\road} &
%     \textbf{\kgen} &
%     \textbf{\kgzh} &
%     \textbf{\kgenzh} &
%     \textbf{\enron} &
%     \textbf{\amazon} &
%     \textbf{\circuit} &
%     \textbf{\ppi} \\
%     \hline
%     \mcsp         & 2.040  & 10.724 & 1.415  & 0.974  & 1.722   & 2.891  & 1.776   & 0.498 \\
%     \mcsprl      & 0.894  & 6.834  & 2.103  & 1.247  & 2.166   & 3.107  & 2.080   & 0.559  \\
%     \hline
%     \gwqap        & 0.548  & 0.834  & 0.546  & 4.692  & 1.041   & 3.419  & 1.550   & 0.546 \\
%     \pca          & 1.152  & 1.797  & 0.967  & 0.897  & 1.739   & 2.725  & 3.792   & 0.636  \\
%     \mcstreemodel & 2.394  & 4.172  & 4.648  & 5.667  & 9.610   & 9.788  & 7.471   & 15.742 \\
%     \hline
%     \randq        & 17.392 & 66.418 & 67.342 & 67.946 & 163.005 & 71.972 & 655.447 & 83.488 \\
%     \mcsrlmodel   & 8.132  & 66.552 & 71.409 & 96.262 & 135.087 & 51.181 & 37.377  & 60.509 \\
%     % \hline
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}

% % \begin{table*}[h]
% % % \small
% %   \begin{center}
% %     \caption{TODO}
% %     \begin{tabular}{l|cccccccc}
% %     \label{table-acc}
% %     \textbf{Method} &
% %     \textbf{\road} &
% %     \textbf{\kgen} &
% %     \textbf{\kgzh} &
% %     \textbf{\kgenzh} &
% %     %\textbf{\facebook} &
% %     \textbf{\enron} &
% %     \textbf{\amazon} &
% %     \textbf{\circuit} &
% %     \textbf{\ppi} \\
% %       \hline
% %       \mcsrlmodel $(N_b = 1; N_d = 10)$ & 115 & 508 & \textbf{513} & \textbf{527} & 519 & \textbf{842} & 3419 & 399 \\
% %       \mcsrlmodel $(N_b = 1; N_d = 20)$ & 131 & 508 & 482 & 521 & \textbf{543} & 791 & 3515 & \textbf{404} \\
% %       \mcsrlmodel $(N_b = 1; N_d = 30)$ & \textbf{149} & \textbf{510} & 484 & 520 & 507 & 784 & \textbf{4219} & 397 \\
% %       \hline
% %       \mcsrlmodel $(N_b = 1; N_d = 10)$ & 115 & 508 & \textbf{513} & \textbf{527} & 519 & \textbf{842} & \textbf{3419} & \textbf{399} \\
% %       \mcsrlmodel $(N_b = 2; N_d = 20)$ & 122 & 494 & 464 & 517 & 540 & 819 & 2206 & 395 \\
% %       \mcsrlmodel $(N_b = 3; N_d = 30)$ & \textbf{155} & \textbf{515} & 500 & 500 & \textbf{1422} & 796 & 2189 & 386 \\
% %     \end{tabular}
% %   \end{center}
% % \vspace*{-6mm}
% % \end{table*}


% \begin{figure}
%      \centering
%      \subfloat[\road]{\includegraphics[width=0.5\textwidth]{vis/Road.png}}
%      \subfloat[\kgen]{\includegraphics[width=0.5\textwidth]{vis/DbEn.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\kgzh]{\includegraphics[width=0.5\textwidth]{vis/DbZh.png}}
%      \subfloat[\kgenzh]{\includegraphics[width=0.5\textwidth]{vis/Dbpd.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\enron]{\includegraphics[width=0.5\textwidth]{vis/Enro.png}}
%      \subfloat[\amazon]{\includegraphics[width=0.5\textwidth]{vis/CoPr.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\circuit]{\includegraphics[width=0.5\textwidth]{vis/Circ.png}}
%      \subfloat[\ppi]{\includegraphics[width=0.5\textwidth]{vis/HPpi.png}}
%      \caption{For each method, we maintain the best solution found so far in each iteration during the search process. We plot the size of the largest extracted common subgraphs found so far vs search iteration count for all the methods across all the datasets. The larger the subgraph size, the better (``smarter'') the model in terms of quickly finding a large MCS solution under limited budget for large graphs.}
%      \label{fig-iter-size}
% \end{figure}


% % \begin{figure}
% % % \vspace{-1.8em}
% %     \centering
% %     \subfloat[On AIDS. Different colors represent different node labels.]
% %     {{\includegraphics[scale=0.37]{vis/Road.png} }}
% %     \vspace{-0.0in}
% %     \centering
% %     \subfloat[On LINUX.]
% %     {{\includegraphics[scale=0.37]{vis/DbEn.png} }}
% %     \vspace{-0.0in}
% %     \centering
% %     \subfloat[On IMDB.]
% %     {{\includegraphics[scale=0.37]{vis/DbZh.png} }}
% %     \vspace{-0.0in}
% %     \caption{Query case studies.}
% %     \label{fig-iter-size}
% % % \vspace{-2.8em}    
% % \end{figure}


% In addition to reaching a larger solution is less iterations, \mcsrlmodel also reaches better solutions with respect to runtime, as shown in Figure~\ref{fig-time-size}. Notice, \mcsrlmodel finds the same large subgraph in 10 minutes as in 7500 iterations. Although per iteration, it is slower than \mcsp per iteration, \mcsrlmodel finds a larger solution in usually less than a minute. Moreover, our implementation can be further optimized. Note, we adapted all baselines to run on Python for fair comparison, and made sure the search iteration counting is consistent across all baselines and the results shown in the main text. At this stage, our main goal is to explore the idea of \textit{\textbf{``learning to search''}}, which has been experimentally verified to be a promising direction of research, and leave the efforts of implementation optimization using various techniques as future focus.

% % Although our goal is to design a model to reach larger solutions in less iterations, and our real running time is slower compared to simpler heuristics-based algorithms, we still compare the subgraph growth vs running time of \mcsp and \mcsrlmodel in Figure~\ref{fig-time-size} under a budget of 10 minutes. Notice, \mcsrlmodel finds the same large subgraph in 10 minutes as in 7500 iterations. Although per iteration, it is slower than \mcsp per iteration, \mcsrlmodel finds a larger solution in usually less than a minute. Moreover, our implementation can be further optimized which can be left as future work. Note that for \mcsprl, it is implemented in C++, and we have currently only adapted \mcsp into our Python framework for a fair real time evaluation. We do make sure the search iteration counting is consistent across the C++ and Python implementations, which is the results shown in the main text. At this stage, our main goal is to explore the idea of \textit{\textbf{``learning to search''}}, which has been experimentally verified to be a promising direction of research, and leave the efforts of implementation optimization using various techniques as future focus.




% \begin{figure}
%      \centering
%      \subfloat[\road]{\includegraphics[width=0.5\textwidth]{vis/Road_time.png}}
%      \subfloat[\kgen]{\includegraphics[width=0.5\textwidth]{vis/DbEn_time.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\kgzh]{\includegraphics[width=0.5\textwidth]{vis/DbZh_time.png}}
%      \subfloat[\kgenzh]{\includegraphics[width=0.5\textwidth]{vis/Dbpd_time.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\enron]{\includegraphics[width=0.5\textwidth]{vis/Enro_time.png}}
%      \subfloat[\amazon]{\includegraphics[width=0.5\textwidth]{vis/CoPr_time.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\circuit]{\includegraphics[width=0.5\textwidth]{vis/Circ_time.png}}
%      \subfloat[\ppi]{\includegraphics[width=0.5\textwidth]{vis/HPpi_time.png}}
%      \caption{For each method, we maintain the best solution found so far in each iteration during the search process. We plot the size of the largest extracted common subgraphs found so far vs the real running time for all the methods across all the datasets. The larger the subgraph size, the better (``smarter'') the model in terms of quickly finding a large MCS solution under limited budget for large graphs.}
%      \label{fig-time-size}
% \end{figure}




% \subsection{Additional Ablation Study}

% Table~\ref{table-abl-ptil} shows that pre-training and imitation learning benefit the performance under four out of the eight datasets. On \enron and \ppi, without pre-training, our model performs better, which may be attributed to the fact that they are dense graphs (Table~\ref{table-test-data}) while the training graphs used in stage 1 are relatively small and sparse (Section~\ref{subsec-cur-learning}).

% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Contribution of pre-training and imitation learning to the performance of \mcsrlmodel. ``no-sup'' denotes the removal of the pre-training stage (The first 3750 iterations: IL; The last 6250 iterations: Normal QDN training); ``no IL'' denotes the removal of the imitation learning stage (The first 3750 iterations: pre-training; The last 6250 iterations: normal DQN training); ``no sup; no IL'' indicates the entire training (10000 iterations) is normal DQN training.}
    
%     \begin{tabular}{l|llllllll}
%     \label{table-abl-ptil}
%     % \multirow{}{} 
%     \textbf{Method}&
%     \textbf{\road} &
%     \textbf{\kgen} &
%     \textbf{\kgzh} &
%     \textbf{\kgenzh} &
%     %\textbf{\facebook} &
%     \textbf{\enron} &
%     \textbf{\amazon} &
%     \textbf{\circuit} &
%     \textbf{\ppi} \\
%     \hline
% \mcsrlmodel (no sup) & 0.557 & 0.957 & 0.946 & 0.904 & \textbf{1.000} & 0.999 & \textbf{1.000} & \textbf{1.000} \\
% \mcsrlmodel (no IL) & \textbf{1.000} & 0.933 & 0.965 & 0.887 & 0.357 & 0.875 & 0.666 & 0.632 \\
% \mcsrlmodel (no sup; no IL) & 0.678 & 0.907 & 0.896 & 0.837 & 0.401 & 0.949 & 0.949 & 0.651 \\
%     \hline
%     \mcsrlmodel & 0.879 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.412 &\textbf{1.000} & 0.855 & 0.688\\
%     \hline
%     \hline
%     \nnodes & 149 & 486 & 465 & 471 & 1318 & 790 & 4112 & 587 \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}





% Table~\ref{table-abl-promise} shows that the promised-based search improves the performance under four out of the eight datasets. For the other four datasets, the performance does not change, indicating that the backtracking to an earlier promising state based on the DQN output at least does not hurt the performance. In the cases like \enron and \ppi, whose average node degrees are large, the promise-based search improves the performance by a large amount, showing the usefulness of the proposed strategy.

% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Contribution of promise-based search (Section~\ref{subsec-backtrack-dqn}) to the performance of \mcsrlmodel. ``no promise'' denotes that the search does not use the proposed promise-based search, i.e. it does not backtrack to an earlier state if the search makes no progress after a certain amount of iterations, and instead, it continues the regular branch and bound search.}
    
%     \begin{tabular}{l|llllllll}
%     \label{table-abl-promise}
%     % \multirow{}{} 
%     \textbf{Method}&
%     \textbf{\road} &
%     \textbf{\kgen} &
%     \textbf{\kgzh} &
%     \textbf{\kgenzh} &
%     %\textbf{\facebook} &
%     \textbf{\enron} &
%     \textbf{\amazon} &
%     \textbf{\circuit} &
%     \textbf{\ppi} \\
%     \hline
%     \mcsrlmodel (no promise) & 0.879 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.412 &\textbf{1.000} & 0.855 & 0.688 \\
%     \hline
%     \mcsrlmodel & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} &\textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
%     \hline
%     \hline
%     \nnodes & 131 & 508 & 482 & 521 & 543 & 791 & 3515 & 404 \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}


% \subsection{Scalability Study}

% \mcsrlmodel can scale to very large graphs containing tens of thousands of nodes. To verify this, we generate 6 large synthetic graphs (3 graph pairs) using the BA, ER, and WS algorithms, each with 10000 nodes, and ran \mcsrlmodel against heuristic-based baselines for 7500 iterations. Our model is superior in all instances, as shown in Table~\ref{table-scal-study}.

% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Results of \mcsrlmodel to even larger networks. Each synthetic dataset consists of one graph pair labeled as $\langle$generation algorithm$\rangle$-$\langle$number of nodes in each graph$\rangle$. For BA graphs, we set the edge density to 4. For ER graphs, we set the edge density to 0.0016. For WS graphs, we set the rewiring probability to 0.2 and ring density to 4.}
    
%     \begin{tabular}{l|lll}
%     \label{table-scal-study}
%     % \multirow{}{} 
%     \textbf{Method}&
%     \textbf{BA-10k} &
%     \textbf{ER-10k} &
%     \textbf{WS-10k} \\
%     \hline
% \mcsp & 0.952 & 0.975 & 0.911 \\
% \mcsprl & 0.964 & 0.975 & 0.911 \\
%     \hline
%     \mcsrlmodel & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
%     \hline
%     \hline
%     \nnodes & 3172 & 2190 & 4839 \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}


% % \mcsrlmodel will retain consistent performance as graph size increases, but heuristic baselines will start to fail, as a smarter policy is required as graph sizes scale up. We validate this claim through constructing 6 new datasets from the circuit dataset, \circuit, sampling isomorphic subgraphs with differing numbers of nodes. In this case, we know the ground truth MCS, which is the whole graph. We ran \mcsrlmodel against heuristic-based baselines for 7500 iterations, and find \mcsrlmodel outperforms heuristic baselines in all experiments, significant performance advantage (~2x performance) begins once graphs are larger than 256 nodes, and our model consistently matches almost the entire graph

% % \begin{table}[h]
% % \small
% %   \begin{center}
% %     \caption{TODO}
    
% %     \begin{tabular}{l|lllllll}
% %     \label{table-abl-ptil}
% %     % \multirow{}{} 
% %     \textbf{Method}&
% %     \textbf{\circuit -128} &
% %     \textbf{\circuit -256} &
% %     \textbf{\circuit -512} &
% %     \textbf{\circuit -1024} &
% %     \textbf{\circuit -2048} &
% %     \textbf{\circuit -4096} &
% %     \textbf{\circuit (4275)} \\
% %     \hline
% % \mcsp & 0.812  & 0.559  & 0.281 & 0.282 & 0.480 & 0.645 & 0.498 \\
% % \mcsprl & 0.812  & 0.559  & 0.269 & 0.432 & 0.476 & 0.633 & 0.583 \\
% %     \hline
% %     \mcsrlmodel & \textbf{1.000} & \textbf{1.000} & \textbf{1.000}  & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
% %     \hline
% %     \hline
% %     \nnodes & 128 & 256 & 509 & 999 & 2040 & 4033 & 3515 \\
% %     \end{tabular}
% %   \end{center}
% % \vspace*{-4mm}
% % \end{table}

% \subsection{Results on Graph Pairs with Known MCS Size Lower Bound}


% To better understand the quality of subgraphs found by \mcsrlmodel, we construct new datasets with known lower bound MCS sizes. This is accomplished through generating 2 new graphs that share a common subgraph from the existing large real-world graph datasets. For each real-world graph, $\mathcal{G}_0$, we randomly extract 3 different subgraphs of the same size, $\mathcal{S}_0$, $\mathcal{S}_1$, and $\mathcal{S}_2$, by running breadth first search from 3 different starting nodes and extracting the explored induced subgraph. To construct a new graph pair, ($\mathcal{G}_1$, $\mathcal{G}_2$), we form $\mathcal{G}_1$ by connecting $\mathcal{S}_0$ to $\mathcal{S}_1$ with 20 random edges and form $\mathcal{G}_2$ by connecting $\mathcal{S}_0$ to $\mathcal{S}_2$ with 20 random edges. Thus, connections between $\mathcal{S}_0$ nodes are the same in both $\mathcal{G}_1$ and $\mathcal{G}_2$, but connections between $\mathcal{G}_1 \setminus \mathcal{S}_0$ and $\mathcal{G}_2 \setminus \mathcal{S}_0$ are different. Notice, the lower bound of MCS size in these new datasets would be $|\mathcal{S}_0|$, and we name the new dataset by adding `ss' to the parent dataset's name.


% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Results on graph pairs with a common core subgraph (lower bound of MCS), with a fixed runtime of 10 minutes.}

    
%     \begin{tabular}{l|llllll}
%     \label{table-acc}
%     \multirow{2}{*}{\textbf{Method}} &
%     \textbf{\road-ss} &
%     \textbf{\kgen-ss} &
%     \textbf{\kgzh-ss} &
%     \textbf{\enron-ss} &
%     \textbf{\amazon-ss} &
%     \textbf{\ppi-ss} \\
%     & 444 & 778 & 762 & 1346 & 1406 & 860 \\
%          \hline
%     \mcsp         & 0.588   & 0.466   & 0.544   & 0.216   & 1.000   & 0.233  
% \\
%     \mcsprl       & 0.588   & 0.466   & 0.544   & 0.214   & 1.000   & 0.233 \\
%     \hline
%     \mcsrlmodel   & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
%     \hline
%     \hline
%     \nnodes & 187     & 388     & 349     & 672     & 702     & 429    \\
%     \textsc{Core (Lower Bound) Size} & 222     & 389     & 381     & 673     & 703     & 430    \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}

